Individual Fairness Guarantees for Neural Networks

We consider the problem of certifying the individual fairness (IF) of feed-forward neural networks (NNs). In particular, we work with the $\epsilon$-$\delta$-IF formulation, which, given a NN and a similarity metric learnt from data, requires that the output difference between any pair of $\epsilon$-similar individuals is bounded by a maximum decision tolerance $\delta \geq 0$. Working with a range of metrics, including the Mahalanobis distance, we propose a method to overapproximate the resulting optimisation problem using piecewise-linear functions to lower and upper bound the NN's non-linearities globally over the input space. We encode this computation as the solution of a Mixed-Integer Linear Programming problem and demonstrate that it can be used to compute IF guarantees on four datasets widely used for fairness benchmarking. We show how this formulation can be used to encourage models' fairness at training time by modifying the NN loss, and empirically confirm our approach yields NNs that are orders of magnitude fairer than state-of-the-art methods.

==> sections/2_problem_statement.tex <==
\section{Individual Fairness}\label{sec:IndFairness}
We develop a framework for the certification of individual fairness of neural networks on regression and binary classification tasks, since these are %generally the tasks of concern 
typically used 
in the fairness literature.
In fact, the former is the learning formalism generally used for ranking systems (e.g.\ select top $k$ students for university admission), while the latter is employed for single application processes (e.g.\ loan applications, or other accept/reject scenarios).\footnote{We remark that the techniques we develop can be generalised to the multi-output case by iteratively applying them to each output component of the NN, at the price of an incrased computational cost.} %\AP{One sentence on why those two cases in particluar}\EB{Added something let me know what you think}
%of the predictions of a  neural networks are fair and use the resulting methods to build deep learning models that are fair by construction.

For an input set $X\subseteq \mathbb{R}^n$, and an output set $Y\subseteq \mathbb{R}$, we consider an $L$ layer fully-connected neural network  (NN) $f^{w} : X\mapsto Y$,  parameterised by a vector of weights  $w \in \mathbb{R}^{n_w}$. 
Specifically,  for  an input point $x \in X$ the NN is defined by the following set of computations, for $i=1,\ldots,L$: 
%
\begin{align}\label{eq:nn}
    &\zeta^{(0)}_j = x_j,\\
    &\phi^{(i)}_j = \sum_{k =1}^{n_{i-1}} W^{(i)}_{jk} \zeta^{(i-1)}_k  + b^{(i)}_{j}, \\ %j=1,\ldots,n_i \\
    &\zeta^{(i)}_j = \sigma^{(i)}\left(\phi^{(i)}_j\right), \quad j=1,\ldots,n_i.
\end{align}
%
Here, $n_i$ is the number of units in the $i$th layer, $W^{(i)}_{jk}$ and  $b^{(i)}_{j}$ are its weights and biases, $\sigma^{(i)}$ is the activation function (e.g.\ ReLU or sigmoid), $\phi^{(i)}$ is the pre-activation value and $\zeta^{(i)}$ is the corresponding activation. 
The output of the NN is the result of these computations, i.e.\ $f^w(x) := \zeta^{(L)}.$ 
%In the regression case $f^w$ directly represents the value of the regression variable, while in the case of binary classification $f^w$ induces a binary classifier $h:\mathbb{R}^n\to\{0,1\}$ such that for a given decision threshold $\eta$ (often taken to be $0.5$) we have that $h(x) = 1$ if $f^w(x)\geq \eta$ and  $h(x) = 0$ otherwise. %$h(x)=\begin{cases}

%Notice our output is a real value, covering the case of regression and binary classification, the value being the probability of the positive class in the latter case.
Individual fairness \citep{Dwork2012FairnessAwareness} considers the behaviour of the NN on ``similar'' individuals.
Similarity is defined according to a problem-dependent input pseudometric, $d_\text{fair}: X \times X  \mapsto \mathbb{R}_{\geq 0}$.
%In particular, we rely on the formalisation of \cite{john2020verifying}. 
%In this paper we aim to develop a framework to certify the fairness of the predictions of a  neural networks are fair and use the resulting methods to build deep learning models that are fair by construction.
%In particular, following \cite{Dwork2012FairnessAwareness}, given appropriately defined distance functions $d_x: \mathbb{R}^n \times \mathbb{R}^n  \mapsto \mathbb{R}_{\geq 0}$, $d_{y}: \mathbb{R} \times \mathbb{R}  \mapsto \mathbb{R}_{\geq 0}$ as well as thresholds $\epsilon>0$ and $\delta >0$ we consider the following notion of individual fairness.
%
\begin{definition}[$\epsilon$-$\delta$-individual fairness \citep{john2020verifying}]\label{def:IndFairness}
Consider $\epsilon \geq 0$ and $\delta \geq 0$. We say that $f^w$ is $\epsilon$-$\delta$-individually fair w.r.t.\ $d_{\text{fair}}$ iff
%\begin{align}\label{eq:eps_delta_def}
% \forall x',x'' \in X \; \text{s.t.} \;    d_{\text{fair}}(x',x'') \leq \epsilon \text{ it holds that } |f^w(x') - f^w(x'')| \leq  \delta.
%\end{align}
\begin{align}\label{eq:eps_delta_def}
 \forall x',x'' \; \text{s.t.} \;    d_{\text{fair}}(x',x'') \leq \epsilon \nonumber \\ \text{ it holds that } |f^w(x') - f^w(x'')| \leq  \delta
\end{align}
\end{definition}
%\LL{An interesting variant, which would allow us to scale to larger systems and problems, could be that where set $X$ is a sampled for an unknown distribution and you want to guarantee the fairness for this distributionally relaxed problem.}
% In particular if $f$ is a classification model, then one could also look for consistency in classification, i.e.\ $f(x') = f(x'')$.
% The extra parameters $\epsion, \delta$ gives us extra flexibility during the analysis.
%
According to Definition~\ref{def:IndFairness}, a model is individually fair if small perturbations (w.r.t.\ to $d_\text{fair}$) of each point in the input space are treated similarly by the neural network.
Notice that  Definition~\ref{def:IndFairness} is a \textit{global} notion, as the condition in Equation \eqref{eq:eps_delta_def} must hold for all the points in the input space $X$.
The choice of the pseudometric $d_\text{fair}$ identifies what individual similarity means in the dataset at hand.
For example, if race were considered a sensitive attribute, $d_\text{fair}$ would assign a distance of zero to two individuals $x'$ and $x''$ which differ only in their race. 
%Furthermore, $d_\text{fair}$ can capture the degree of correlation that the remaining features might w.r.t.\ the sensitive attributes (e.g., ZIP code might be related to race \citep{missing}).
In particular, although our method can be generalised to different notions, we focus on the following representative similarity metrics from the literature \citep{john2020verifying,ruoss2020learning,mukherjee20simple,yurochkin2020training,ilvento19metric} (additional details are given in the Supplementary Material).\\
%We learn these metrics from the data themselves by using the methods highlighted in \citep{missing,missing}. 
 % \AP{We could also move all these discussion on the metric to the supplementary if we need space...}.\LL{I like them in here, it gives some context.}
\textbf{Weighted $\ell_p$ Metric.}
In this case $d_{\text{fair}}(x',x'')$ is defined as a weighted version of an $\ell_p$ metric, as in:

$d_{\text{fair}}(x',x'') = \sqrt[p]{\sum_{i=1}^n \theta_i |x'_i - x''_i|^p}  $.
Intuitively, we set the weights $\theta_i$ related to sensitive features (e.g., race or sex) to zero, so that two individuals are considered \textit{similar} if they only differ with respect to one of the sensitive features.
Additionally, the weights $\theta_i$ for the remaining features can be tuned accordingly to their degree of correlation to the sensitive features.\\% (e.g., ZIP code might be related to race in certain circumstances \citep{missing}).
\textbf{Mahalanobis Metric.}
In this case we have $d_{\text{fair}}(x',x'')  = \sqrt{(x'-x'')^T S (x'-x'')}$, for a given positive semi-definite (SPD) matrix $S$.
Intuitively, the Mahalanobis distance generalises the $\ell_2$ metric by also taking into account the intra-correlation between features that captures the latent dependency w.r.t.\ the sensitive features.\\
\textbf{Feature Embedding Metric.} 
The metric is computed on an embedding, so that $d_{\text{fair}}(x',x'') = \hat{d}(\varphi(x'),\varphi(x''))$, where $\hat{d}$ is either the Mahalanobis or the weighted  $\ell_p$ metric, and  $\varphi$ is a feature embedding map. These allow for greater modelling flexibility, at the cost of reduced interpretability.
%These allows for greater flexibility in dealing \LL{There is a sentence missing in here?}

%\LL{Describe the distance functions we use in here.}
%\EB{Re my convo with Andrea: we can stay fairly general and state that we focus in our experiment on a mahalanobis distance. A nice extra could be to have some experiments with something like a weighted LP norm like that used by \cite{john2020verifying}}.

%We should also note also that Definition \ref{def:IndFairness} is a global notion as Condition \eqref{eq:eps_delta_def} must holds for all samples in the input space. Nevertheless, we should stress that Definition \ref{def:IndFairness} can be relaxed by having Condition \ref{eq:eps_delta_def} to hold for all $x',x''\in \bar{X}\subseteq X.$

\subsection{Problem Formulation}
We formalise two problems concerning individual fairness in NNs, respectively concerning certification and training of fair neural networks.
%the first one regarding verification the second one regarding training of fair neural networks.
\begin{problem}[Fairness Certification]\label{prob:certification}
Given a neural network $f^w$, a similarity metric $d_{\text{fair}}$ and a distance threshold $\epsilon \geq 0$, compute 
\begin{align*}
    \delta_{\max}=\max_{\substack{ x',x'' \in X \\  d_{\text{fair}}(x',x'') \leq \epsilon}} |f^w(x') - f^w(x'')|.
\end{align*}
\end{problem}
%
Problem \ref{prob:certification} seeks to compute the maximum change in the NN output for any two points in the considered input domain $X$ whose fair distance is no more than $\epsilon$. One can then compare the computed $\delta_{\max}$ with a given threshold $\delta$ to check if $f^w$ is $\epsilon$-$\delta$-individually fair as per Definition \ref{def:IndFairness}. 
%In the following problem instead of simply checking if a NN is fair, we seek to train NNs that are fair by construction.
While Problem~\ref{prob:certification} is concerned with the verification of individual fairness in an already trained NN, we can also employ our methodology to modify the NN's loss function to take into account individual fairness at training time.
To do so, call $\mathcal{D}=\{(x_i,y_i), i\in \{1,...,n_{d} \}\}$ the training dataset and  $L(f^w(x),y)$ the loss function used for training the NN (e.g.\ cross-entropy).
Similarly to the approaches for adversarial learning \citep{goodfellow2014explaining}, we modify the training loss to balance between the  model fit and individual fairness computed locally for each point in the training set.  
%
\begin{problem}[Fairness Training]\label{prob:training}
Consider a NN architecture $f^w$, a similarity metric $d_{\text{fair}}$ and a distance threshold $\epsilon \geq 0$. Let $\lambda \in [0,1]$ be a constant, then, the $\epsilon$-individual fairness training problem is defined as the problem of finding the set of weights $w^{\text{fair}}$, such that:
\begin{align}
\begin{split}
&L_{\text{fair}}(f^w(x_i),y_i,f^w(x^*_i))      =  \\
              &\qquad \lambda L(f^w(x_i),y_i) + (1-\lambda) | f^w(x_i) - f^w(x^*_i) | \label{eq:modified_loss} 
%   &L_{\text{fair}}(f^w(x_i),y_i)      = \lambda L(f^w(x_i),y_i) \\
%               &\qquad \qquad \qquad \qquad + (1-\lambda) | f^w(x_i) - f^w(x^*_i) | \label{eq:modified_loss} 
\end{split}\\
\begin{split}
&w^{\text{fair}}   = \argmin_{w}\sum_{i = 1}^{n_d} L_{\text{fair}}(f^w(x_i),y_i)  \nonumber
\end{split}
%    &\begin{split}
%         &L_{\text{fair}}(f^w(x_i),y_i) = \lambda L(f^w(x_i),y_i) \nonumber \\
%         &+ (1-\lambda) | f^w(x_i) - f^w(x^*_i) | \label{eq:modified_loss} \\
%    \end{split}\\
%    &w^{\text{fair}} = \argmin_{w}\sum_{i = 1}^{n_d} L_{\text{fair}}(f^w(x_i),y_i)  \nonumber
\end{align}
where $x^*_i=\argmax_{x \in X \, s.t.\, d_{\text{fair}}(x_i,x) \leq \epsilon} |f^w(x_i) - f^w(x)|$. % Note that the difference between the $L^{\text{fair}}$ maximization problem and that of certification is the existence of a fixed $x$ coming from the dataset. %\LL{Need to be careful in here as they may have different scale, so we may need to normalize. Other approach would be to just add a global term for $L^{fair}$ }.
\end{problem}
%
In Problem~\ref{prob:training} we seek to train a NN that not only is accurate, but whose predictions are also fair according to Definition~\ref{def:IndFairness}. Parameter $\lambda$ balances between accuracy and fairness. In particular, for $\lambda=1$ we recover the standard training approach where we do not account explicitly for fairness, while for $\lambda=0$ we only consider fairness.
Note that the fairness correction term does not depend on the ground truth label but only on the maximum variation between similar individuals.
%\LL{We could emphasize that the correction term is independent of the training label}
%Note also that the loss modification, i.e.\  $(1-\lambda) | f^w(x) - f^w(x^*) |$, does not depend on the training label, but just on the output difference in all the points in a $d_{\text{fair}}-$ball around each data point.
%This is a key difference compared to standard approaches for adversarial training for NN classifiers \citep{madry2017towards,wicker2021bayesian}, where the goal is to have all the points in the ball to be in the same class.  

%\AP{I have commented the previous version out below of this comment in the source file for readability.}
\iffalse
\section{Individual Fairness}

The theoretical definition of individual fairness is given in the original paper by \cite{Dwork2012FairnessAwareness} as the following \textit{(D, d)-Lipschitz} property:\LL{Need to be clearer on how $d_x$ and $d_y$ are defined.}
\begin{align}\label{eq:lipz_def}
   \forall x',x'' \in T \implies d_y(f(x') - f(x'')) \leq d_x(x',x'')
\end{align}

given a decision model $f : \mathbf{R}^{n} \rightarrow \mathbf{R}$, an output distance metric $d_y$ and an input distance (or fair distance) metric $d_x$. Intuitively this is stating that two \textit{comparable} inputs must be treated similarly by the decision model. We say \textit{comparable} and not similar, because, despite a superficial likeness to the definition of robustness, there are two key differences between the two properties. Firstly, this is a \textit{global} property \LL{Well, global depends on how you define T. I would instead first define the neural network and then simply assume that 1 must all for all the inputs.}, that needs to hold over the entire input domain $T$. Secondly, the fair distance metric $d_x$ is generally more complicated than a simple $L^p$-norm (normally used for robustness), since it encapsulates our understanding of the fairness related interactions between different inputs features.

The fair distance metric is in fact a core component of this definition. It is a well-studied fact in the fairness literature (\cite{Pedreshi2008DiscriminationDataMining}, \cite{Udeshi2018AutomatedTesting}) that simply removing sensitive features (also referred to as sensitive attributes) from the data prior to training is not a sufficient strategy to obtain a fair classifier, since there might be other features that are strongly correlated with those removed (e.g. ZIP code might be correlated with ethnicity \EB{Should maybe have a reference for this example}). The metric should account for the degree of correlation of each feature to any sensitive features, and consequently affect the resulting distance. This is to say that, comparatively, data points differing in features correlated to sensitive attributes should be less distant than data points differing in uncorrelated features. Two individuals differing only in their sensitive features should have a fair distance of zero.

The decision functions studied in this paper are those represented by feed-forward neural networks. These are expected to have input features of two kinds: normalised (in $[0,1]$) continuous features, and categorical features, initially one-hot encoded as integer $0,1$ values. The hidden layers are assumed to use ReLU activation functions, and for classification tasks we assume the use of the sigmoid function. As it is standard practice in the fairness literature, we focus on binary classification, since the fairness concerns usually arise from one output option being preferable to the other.

% In this work we focus on training and verification of individual fairness on feed-forward neural networks. We express such networks as a function $y = f(x)$ with X and Y being the domains of the input and output

% \textbf{Allowed input domain and concept of features:} The input is an array of either real values or one-hot encoded categorical features. In practice during training and verification we treat them as real values, with added constraints.

% These have layers, separated by activation functions. We consider two main activation functions. ReLU after each hidden layer. In case of a classification problem we use a sigmoid function. We focus on binary classification as it is standard practice in the fairness literature. This makes sense as you consider one outcome to be more desirable than the other, which is less directly applicable as a concept to multiclass classification.

\section{Problem Formulation}\label{sec:probFormulation}
%\LL{The metric we employ can be described either in here or in the previous Section.}

%\LL{Here describe our problem formulation. I expect this to be divided in two sub-problems: verification and training of fair models.}

In our work, we use the following definition of individual fairness (similar to the one used by \cite{john2020verifying}), as it's more amenable to optimisation than the original property proposed by \cite{Dwork2012FairnessAwareness}:
\begin{align}\label{eq:eps_delta_def}
 \forall x',x'' \in T \; \text{s.t.} \;    d_{\text{fair}}(x',x'') \leq \epsilon \implies |f(x') - f(x'')| \leq  \delta
\end{align}
% In particular if $f$ is a classification model, then one could also look for consistency in classification, i.e.\ $f(x') = f(x'')$.
% The extra parameters $\epsion, \delta$ gives us extra flexibility during the analysis.
This is stating that the output given by a model to any two input points within fair distance $\epsilon$ should differ at most by $\delta$. In the case of regression the two final logit values will be compared. In case of classification it will be the difference in the output of the sigmoid, i.e. the classification confidence.

Importantly, we focus exclusively on metrics taking the form of a Mahalanobis distance, i.e. $d_{\text{fair}}(x',x'') = \sqrt{(x'-x'')^T S (x'-x'')}$. The reason for this choice is twofold. Firstly, to benefit from greater expressivity than simpler weighted $L_p$-norms used in other work (e.g. \cite{john2020verifying}, especially when handling tabular datasets where working with this kind of metric is practical. 
Secondly, we benefit from recent research on data-driven fair distance metrics
(\cite{yurochkin2020training}, \cite{mukherjee20simple}, \cite{ilvento19metric}). We generate a fair metric from auditing data as follows. Assuming tabular data, we expect as input the subset of sensitive features $K$ (\EB{Currently we only cater for categorical/discrete sensitive features}). We then use the non-sensitive features to predict the value of each sensitive feature, fitting a softmax regression model for each:

\begin{align*}
    \textbf{P}(K_i = l | X_i) = \frac{\exp{(a^{T}_{l}X_i + b_{l}})}{\sum_{l=1}^{k} \exp{(a^{T}_{l}X_i + b_{l}})},\; l=1,...,k
\end{align*}

We stack the weights of each model, and then compute the span of the resulting matrix, to obtain the sensitive subspace. We find its orthogonal projector $S = I - P_{\text{ran(A)}}$ (where $A = [a_1, ..., a_k]$) which we use to define the distance metric above.

However, while throughout the paper we refer to a distance metric of this form, much of the methodology later presented does not strictly depend on it. In fact, it could be adapted to work with a wider variety of norms (\EB{Maybe for Andrea, what would you say are the minimum requirements we have for the distance metric? If we have any it would be useful to state it here})

\textbf{Verification}

We define verification of individual fairness on a neural network as a constrained optimisation problem, expressed as:
\begin{align*}
    \max_{x',x'' \in T}& f(x') - f(x'') \\
    \text{subject to}& \quad  d_{\text{fair}}(x',x'') \leq \epsilon.
\end{align*}

% Where $x', x''$ are any two values in T, the given accepted domain over our input space.
We are given T, the accepted domain over our input space from which to draw $x',x''$, the fair distance metric $d_{\text{fair}}$, or in our specific case the matrix $S$, which can be learnt from test data, and $\epsilon$. The returned value is then be compared to the original $\delta$ to establish if the model passes verification or not. Since the optimisation spans across both $x',x''$ this is providing global guarantees of individual fairness over the whole input space. Furthermore, when impractical to complete the optimisation problem, a lower bound is returned, so the results provide strong guarantees.

% we get back the maximum difference (or a lower bound) in output within an $\epsilon$\textit{-neighbourhood} \EB{Not sure how people feel about this term. I came up with it because it's not quite a ball, and didn't know what to call it}, and whether this is within $\delta$. This is a global property, so any pair of inputs within fair distance $\epsilon$ is considered during verification.

\textbf{Training}

We take a classical ERM adversarial approach to the problem of training an individually fair model. Inspired by \cite{madry2017towards}, we define the population risk $\mathbb{E_{\textit{D}}} [L]$ incorporating an individual fairness adversary:

\begin{align*}
    \min_{\theta \in \Theta} \mathbb{E}_{(x,y) \sim \textit{D}} [\max_{d_{\text{fair}}(x, x') < \epsilon} L(\theta, x', y)]
\end{align*}

where $\Theta$ is the class of parameters available to our network, $L$ is a loss function, and $(x, y)$ is a training input and label pair drawn from the training distribution $D$. Intuitively we are trying to find a set of parameters for our model that minimises the loss over adversarial examples identified by the adversary.

In this setting, the attack model, defined as in \cite{madry2017towards} as a precise definition of the attacks our model should be resistant to, is defined as a set of allowed perturbation, corresponding to the points within $\epsilon$ fair distance from our training examples.

In contrast to previous work, where the adversary generates examples using projected gradient descent (PGD) on a negative loss function, of the form:

\begin{align*}
    x^{t+1} = \Pi_{x+S} (x^{t} + \alpha \text{sgn} (\nabla_{x} L(\theta, x, y)))
\end{align*}

our adversary uses MILP local optimisation. Inspired by work on adversarial strategies to train individually fair neural networks (e.g. \cite{yurochkin2020training}), we define a training protocol that at some point during training, for each training point $x$ it solves the following local problem:

\begin{align*}
    \max_{x' \in T}& f(x) - f(x') \\
    \text{subject to}& \quad  d_{\text{fair}}(x,x') \leq \epsilon.
\end{align*}

This finds the $x'$ point within $\epsilon$ fair distance of the original data point with the largest difference in output. $x'$ is then used with the original label of $x$ to steer training towards individual fairness.

\fi
